Unlocking the Edge deployment and ondevice acceleration of multi-LoRA enabled one-for-all foundational LLM

Deploying large language models (LLMs) on smartphones poses significant engineering challenges due to stringent constraints on memory, latency, and runtime flexibility. In this work, we present a hardware-aware framework for efficient on-device inference of a LLaMA-based multilingual foundation model supporting multiple use cases on Samsung Galaxy S24 and S25 devices with SM8650 and SM8750 Qualcomm chipsets respectively. Our approach integrates application-specific LoRAs as runtime inputs to a single frozen inference graph, enabling dynamic task switching without recompilation or memory overhead. We further introduce a multi-stream decoding mechanism that concurrently generates stylistic variations - such as formal, polite, or jovial responses - within a single forward pass, reducing latency by up to 6x. To accelerate token generation, we apply Dynamic Self-Speculative Decoding (DS2D), a tree-based strategy that predicts future tokens without requiring a draft model, yielding up to 2.3x speedup in decode time. Combined with quantization to INT4 and architecture-level optimizations, our system achieves 4-6x overall improvements in memory and latency while maintaining accuracy across 9 languages and 8 tasks. These results demonstrate practical feasibility of deploying multi-use-case LLMs on edge devices, advancing the commercial viability of Generative AI in mobile platforms.

==> section/8_PULSE_Tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

% This is Table 1.
\begin{table}[h]
% \captionsetup{justification=centering}
\caption{PULSE Table 1}
\label{tab:PULSE_Table_1}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{D6DCE5}}c |
>{\columncolor[HTML]{DEEBF7}}c |
>{\columncolor[HTML]{DEEBF7}}c 
>{\columncolor[HTML]{DEEBF7}}c |
>{\columncolor[HTML]{DEEBF7}}c |
>{\columncolor[HTML]{DEEBF7}}c |
>{\columncolor[HTML]{DEEBF7}}c |}
\hline
\cellcolor[HTML]{D6DCE5} & \cellcolor[HTML]{D6DCE5} & \multicolumn{2}{c|}{\cellcolor[HTML]{D6DCE5}\begin{tabular}[c]{@{}c@{}}Speed Up \\    \\ (TPI / BE)\end{tabular}} & \cellcolor[HTML]{D6DCE5} & \cellcolor[HTML]{D6DCE5} & \cellcolor[HTML]{D6DCE5} \\ \cline{3-4}
\multirow{-2}{*}{\cellcolor[HTML]{D6DCE5}Method} & \multirow{-2}{*}{\cellcolor[HTML]{D6DCE5}# of Draft tokens} & \multicolumn{1}{c|}{\cellcolor[HTML]{D6DCE5}Avg.} & \cellcolor[HTML]{D6DCE5}Max & \multirow{-2}{*}{\cellcolor[HTML]{D6DCE5}\begin{tabular}[c]{@{}c@{}}Params \\    \\ (M)\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{D6DCE5}\begin{tabular}[c]{@{}c@{}}RoM   (MB)\\    \\ w-INT8\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{D6DCE5}Remarks} \\ \hline
BiTA & 2 & \multicolumn{1}{c|}{\cellcolor[HTML]{DEEBF7}~2X} & NA & 0.29 & ~0.3 & NA \\ \hline
Eagle & 5 & \multicolumn{1}{c|}{\cellcolor[HTML]{DEEBF7}3.17x} & NA & 99 & 95 & NA \\ \hline
Pulse & 4 & \multicolumn{1}{c|}{\cellcolor[HTML]{DEEBF7}3.26x} & 4.42x & 10.2 & 9.72 & \cellcolor[HTML]{DEEBF7} \\ \cline{1-6}
Pulse & 5 & \multicolumn{1}{c|}{\cellcolor[HTML]{DEEBF7}3.65x} & 5.17x & 11.9 & 11.2 & \cellcolor[HTML]{DEEBF7} \\ \cline{1-6}
Pulse & 10 & \multicolumn{1}{c|}{\cellcolor[HTML]{DEEBF7}5.31x} & 8.75x & 20.8 & 19.62 & \multirow{-3}{*}{\cellcolor[HTML]{DEEBF7}\begin{tabular}[c]{@{}c@{}}Trained   on 3.5 Rotated Gauss-L model, No LoRA,   Summarization   (En) on CNN-DM dataset.   80K  data points on 24 A100-hours.   \\      Tested   on 50 prompts, 1024 Context length.  \\ No Draft tree,   i.e. all 1s as configuration. With tree, results can improve further.\end{tabular}} \\ \hline
\end{tabular}%
}
\end{table}

==> section/9_implementations_suggestions.tex <==




1. GS24, GS25, GS26 -> Gauss Model Information
    1.1 Architecture details
    1.2 Paramater details
2. LoRas & usecase informations.
3. 
